On the adaptive Levin method

The Levin method is a well-known technique for evaluating oscillatory integrals, which operates by solving a certain ordinary differential equation in order to construct an antiderivative of the integrand. It was long believed that this approach suffers from "low-frequency breakdown," meaning that the accuracy of the calculated value of the integral deteriorates when the integrand is only slowly oscillating. Recently presented experimental evidence, however, suggests that if a Chebyshev spectral method is used to discretize the differential equation and the resulting linear system is solved via a truncated singular value decomposition, then no low-frequency breakdown occurs. Here, we provide a proof that this is the case, and our proof applies not only when the integrand is slowly oscillating, but even in the case of stationary points. Our result puts adaptive schemes based on the Levin method on a firm theoretical foundation and accounts for their behavior in the presence of stationary points. We go on to point out that by combining an adaptive Levin scheme with phase function methods for ordinary differential equations, a large class of oscillatory integrals involving special functions, including products of such functions and the compositions of such functions with slowly-varying functions, can be easily evaluated without the need for symbolic computations. Finally, we present the results of numerical experiments which illustrate the consequences of our analysis and demonstrate the properties of the adaptive Levin method.

==> figures.tex <==
%% \vfil\eject

%% \begin{figure}[!h]
%% \hfil
%% \includegraphics[width=.40\textwidth]{elemplot1-err.pdf}
%% \hfil
%% \includegraphics[width=.40\textwidth]{elemplot1-time.pdf}
%% \hfil


%% \hfil
%% \includegraphics[width=.40\textwidth]{elemplot2-err.pdf}
%% \hfil
%% \includegraphics[width=.40\textwidth]{elemplot2-time.pdf}
%% \hfil

%% \hfil
%% \includegraphics[width=.40\textwidth]{elemplot3-err.pdf}
%% \hfil
%% \includegraphics[width=.40\textwidth]{elemplot3-time.pdf}
%% \hfil

%% \hfil
%% \includegraphics[width=.40\textwidth]{elemplot4-err.pdf}
%% \hfil
%% \includegraphics[width=.40\textwidth]{elemplot4-time.pdf}
%% \hfil


%% \caption{\small
%% The results of the experiment of Section~\ref{section:experiments:elem}.
%% The first row of plots pertains to the integral $I_1$, the second to $I_2$
%% and so on.  Each plot on the left gives the error in the value of the integral
%% computed via the adaptive Levin method as a function of $\lambda$, while
%% each plot on the right gives the running time in milliseconds as a function
%% of $\lambda$.
%% }
%% \label{figure:elemplots1}
%% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \vfill\eject


%% \begin{table}[h!]
%% \center
%% \input{gausstable1.tex}
%% \caption{\small
%% The results of the experiment of Section~\ref{section:experiments:gauss}
%% in which the performance of the adaptive Levin method was compared with the 
%% performance of an adaptive Gaussian quadrature scheme.    Each row corresponds
%% to one of the integrals $I_5(\lambda)$, $I_6(\lambda)$, $I_7(\lambda)$ or $I_8(\lambda)$
%% and to one range of values of $\lambda$.
%% The average time taken by the adaptive Levin method and by an adaptive Gaussian quadrature
%% scheme, the ratio
%% of the average time taken by the adaptive Gaussian quadrature algorithm to the average time taken by the
%% adaptive Levin method, and the
%% maximum observed difference in the values of the integrals computed using each method  are reported.
%% }
%% \label{table:gauss:table1}
%% \end{table}


%% \vfil\eject

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

%% \begin{figure}[h!]

%% \hfil
%% \includegraphics[width=.44\textwidth]{saddleplot1-ints.pdf}
%% \hfil
%% \includegraphics[width=.44\textwidth]{saddleplot2-ints.pdf}
%% \hfil
%% \hfil

%% \hfil
%% \includegraphics[width=.44\textwidth]{saddleplot1-errs.pdf}
%% \hfil
%% \includegraphics[width=.44\textwidth]{saddleplot2-errs.pdf}
%% \hfil


%% \hfil
%% \includegraphics[width=.44\textwidth]{saddleplot3-ints.pdf}
%% \hfil
%% \includegraphics[width=.44\textwidth]{saddleplot4-ints.pdf}
%% \hfil

%% \caption{\small
%% The results of the experiment of Section~\ref{section:experiments:saddle}.
%% The plots in the first row give the number of subintervals in the adaptive discretization of $[-1,1]$ formed
%% in the course of evaluating $I_9(\lambda,m)$ as a function of $\lambda$ for $m=2,3,4,5$; those in the second 
%% give the absolute error in the calculated error in the 
%% value  of $I_9(\lambda,m)$ as a  function of $\lambda$ for $m=2,3,4,5$;
%% and the plots in the third row show  the number of subintervals
%% in the adaptive discretization of $[-1,1]$ as a function of $m$ for
%% $\lambda=10^2, 10^3, 10^4, 10^5$.
%% The plots in the column on the left concern experiments executed with
%% the precision parameter  $\epsilon$ taken to be  $10^{-7}$,
%% while those on the right correspond to $\epsilon = 10^{-12}$.
%% }
%% \label{figure:saddleplot1}
%% \end{figure}

%% \vfil\eject

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%555

%% \begin{figure}[!t]
%% \hfil
%% \includegraphics[width=.40\textwidth]{besplot1-err.pdf}
%% \hfil
%% \includegraphics[width=.40\textwidth]{besplot1-time.pdf}
%% \hfil


%% \hfil
%% \includegraphics[width=.40\textwidth]{besplot2-err.pdf}
%% \hfil
%% \includegraphics[width=.40\textwidth]{besplot2-time.pdf}
%% \hfil

%% \hfil
%% \includegraphics[width=.40\textwidth]{besplot3-err.pdf}
%% \hfil
%% \includegraphics[width=.40\textwidth]{besplot3-time.pdf}
%% \hfil

%% \hfil
%% \includegraphics[width=.40\textwidth]{besplot4-err.pdf}
%% \hfil
%% \includegraphics[width=.40\textwidth]{besplot4-time.pdf}
%% \hfil


%% \caption{\small
%% The results of the experiment of Section~\ref{section:experiments:bes}.
%% The first row of plots concerns the integral $I_{10}$.
%% The graph on the left displays the absolute error in the computation of $I_{10}(\nu)$
%% as a function of the order $\nu$ while the graph on the right
%% gives the times required to compute $I_{10}(\nu)$ and the necessary phase function
%% as functions of $\nu$.  Rows $2$, $3$ and $4$ give the results for 
%% $I_{11}(\lambda)$ $I_{12}(\lambda)$ and $I_{13}(\lambda)$, respectively.
%% In each row, the plot on the left gives the absolute error in the calculation
%% of the integral as a function of $\lambda$ and the plot on the right shows
%% the time required to compute the integral via the adaptive Levin method
%% as a function of $\lambda$.
%% }
%% \label{figure:besplots1}
%% \end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% %% \vfil\eject


%% %% \begin{figure}[!h]

%% %% \hfil
%% %% \includegraphics[width=.40\textwidth]{alfplot1-err.pdf}
%% %% \hfil
%% %% \includegraphics[width=.40\textwidth]{alfplot1-time.pdf}
%% %% \hfil

%% %% \hfil
%% %% \includegraphics[width=.40\textwidth]{alfplot2-err.pdf}
%% %% \hfil
%% %% \includegraphics[width=.40\textwidth]{alfplot2-time.pdf}
%% %% \hfil

%% %% \hfil
%% %% \includegraphics[width=.40\textwidth]{alfplot3-err.pdf}
%% %% \hfil
%% %% \includegraphics[width=.40\textwidth]{alfplot3-time.pdf}
%% %% \hfil


%% %% \caption{\small
%% %% The results of the experiment of Section~\ref{section:experiments:alf}.
%% %% The plots in the first row give the error in the calculated value of  $I_{15}(m+\nu,m)$
%% %% and the time required to calculate it via the adaptive Levin method
%% %% as functions of $\nu$ for $m=10, 10^2, 10^3, 10^4$.
%% %% The plots in the second row give the same information for $I_{16}(m+\nu,m)$ and 
%% %% those in the third row pertain to $I_{17}(m+\nu,m)$.
%% %% }
%% %% \label{figure:alfplots1}

%% %% \end{figure}

%% \vfil\eject


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%555555


%% \begin{figure}[!h]

%% \hfil
%% \includegraphics[width=.35\textwidth]{modalplot1-err.pdf}
%% \hfil
%% \includegraphics[width=.35\textwidth]{modalplot1-time.pdf}
%% \hfil

%% \hfil
%% \includegraphics[width=.35\textwidth]{modalplot2-err.pdf}
%% \hfil
%% \includegraphics[width=.35\textwidth]{modalplot2-time.pdf}
%% \hfil

%% \caption{\small
%% The results of the first experiment of Section~\ref{section:experiments:modal}.
%% The plot on the left-hand side of  the first row gives the absolute error in the calculated value of  $I_{19}(\kappa,m,\alpha)$
%% as a function of $m$ for four values of $\kappa$ in the case $\alpha=0.5$.
%% The plot on the right-hand side of  the first row gives the time required to calculate  $I_{19}(\kappa,m,\alpha)$
%% via the adaptive Levin method as a function of $m$ for four values of $\kappa$ in the case $\alpha=0.5$.
%% The plots in the second row give analagous data in the event $\alpha=0.99$.
%% }
%% \label{figure:modalplots1}
%% \end{figure}


%% \begin{figure}[!b]
%% \hfil
%% \includegraphics[width=.35\textwidth]{modalplot3-err.pdf}
%% \hfil
%% \includegraphics[width=.35\textwidth]{modalplot3-time.pdf}
%% \hfil


%% \hfil
%% \includegraphics[width=.35\textwidth]{modalplot4-err.pdf}
%% \hfil
%% \includegraphics[width=.35\textwidth]{modalplot4-time.pdf}
%% \hfil

%% \caption{\small
%% The results of the second experiment of Section~\ref{section:experiments:modal}.
%% The plot on the left-hand side of  the first row gives the absolute error in the calculated value of  $I_{19}(\kappa,m,\alpha)$
%% as a function of $\kappa$ for four values of $m$ in the case $\alpha=0.5$.
%% The plot on the right-hand side of  the first row gives the time required to calculate  $I_{19}(\kappa,m,\alpha)$
%% via the adaptive Levin method as a function of $\kappa$ for four values of $m$ in the case $\alpha=0.5$.
%% The plots in the second row give analagous data in the event $\alpha=0.99$.
%% }
%% \label{figure:modalplots2}
%% \end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%555555
%% \vfil\eject


%% \begin{figure}[!h]


%% \hfil
%% \includegraphics[width=.40\textwidth]{saddleplot11-time.pdf}
%% \hfil
%% \includegraphics[width=.40\textwidth]{saddleplot10-time.pdf}
%% \hfil

%% \hfil
%% \includegraphics[width=.40\textwidth]{saddleplot11-ints.pdf}
%% \hfil
%% \includegraphics[width=.40\textwidth]{saddleplot10-ints.pdf}
%% \hfil

%% \hfil
%% \includegraphics[width=.40\textwidth]{saddleplot11-errs.pdf}
%% \hfil
%% \includegraphics[width=.40\textwidth]{saddleplot10-errs.pdf}
%% \hfil




%% \caption{\small
%% The results of the experiments of Section~\ref{section:experiments:saddle2}.
%% The plots in the first row give
%% the   time taken by the adaptive Levin method as a function of $\lambda$ for the various values
%% of $m$ considered.    Those in the second row give the 
%% number of intervals  in the adaptively determined subdivision of $[-1,1]$ used to compute the integral
%% $I_20$ as a function of $\lambda$ for the values of $m$ considered.
%% The third row of plots give
%% the error in the calculated value of  $I_{20}(\lambda,m)$ 
%%  as a function of $\lambda$ for $m=15,20,25,30,35,40,45,50$.
%% }
%% \label{figure:saddleplots2}
%% \end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


